Human-in-the-Loop through Chain-of-Thought

While the emergence of powerful language models along with Chain-of-thought prompting has made automation more and more omnipresent, it sometimes demonstrates its weakness in long-term or multi-step logical reasoning. For example, users don't always get desirable answers for complex mathematical problems without human involvement. Against this background, we present the Manual Correction System (MCS) -- a human-in-the-loop system enhanced by Chain-of-Thought prompting, which explores how manual correction of sub-logics in rationales can improve LLM's reasoning performance. Moving one step forward, considering a system with human-in-the-loop involves more than having humans improve performance but also controlling the cost. Therefore, we post a Cost-utility Analysis Model for Human-in-the-Loop systems (CAMLOP) based on classical economics theory to analyze, quantify and balance the utility and the corresponding cost. We conduct experiments of MCS and CAMLOP with twelve datasets. A significant advantage w.r.t cost and utility proves its superiority over strong baselines.

==> files/temp/temp.tex <==

\section{Experiments}
\label{sec:experiments}
% We conducted a series of experiments to compare the proposed \model method with existing baselines on a range of arithmetic, commonsense reasoning benchmarks, and symbolic reasoning tasks. 
% It can be observed that the \model generally boosts the strong baselines. A significant advantage w.r.t cost and utility proves our \model's superior over baselines. 

\subsection{Experiment Setup}

% 需要重新写，我模仿self-consistency这篇论文的
\paragraph{Tasks and datasets.} 
% We conducted experiments on the following reasoning benchmarks.
For arithmetic reasoning tasks, we conducted a series of experiments on the Math Word Problem Repository \citep{amini2019mathqa}, including AddSub \citep{hosseini2014learning}, MultiArith \citep{roy2016solving}, Singleeq \citep{koncel2015parsing} and Singleop \citep{kushman2014learning}. We also included  ASDiv \citep{miao2021diverse}, AQUA-RAT \citep{miao2021diverse}, GSM8K \citep{cobbe2021training}, and ASDiV \citep{patel2021nlp}.
% The last four are recently published benchmarks. 
For commonsense reasoning tasks, we used CommonsensQA\citep{talmor2018commonsenseqa} and StrategyQA\citep{geva2021did}. For symbolic reasoning tasks, we used Last Letter Concatenation and Coinflip\citep{wei2022chain}.

\paragraph{Models and scales.} 
We use GPT-3 \citep{ouyang2022training,brown2020language}
\footnote{The \texttt{text-davinci-002} version is InstructGPT. We use the \textit{text-davinci-002} version of GPT-3 to finish all the experiments.} 
with 175-billion parameters as the LLM. 
More details are provided in Appendix~\ref{apdx:experiment_details}.
For our methods, we provide the following two variants.
\begin{itemize}[wide, labelwidth=!, labelindent=15pt]
    \item \textit{\model.} \model is the result of manual correction for the top40\% CoT predictions ranked out using diversity metrics. We provide an ablation study in Sec.~\ref{paragraph:ablation-diversity-metrics-ratio} to show the results of different ratio selections for diversity metrics.
    \item \textit{\model+Self-consistency.} \model + Self-consistency is the result of combining marginalizing out the sampled rationales with manual correction for the top40\% CoT predictions ranked out using diversity metrics. In practice, we use Self-consistency to get answer by majority vote, and then we use \model to manually correct incorrect sub-logics with Diversity Entropy calculated based on the decoded reasoning paths.
\end{itemize}
\paragraph{Sampling scheme.}  To sample diverse rationales, we followed similar settings to those used in Wang et al. (2022) \citet{wang2022self} for the open-text generation. We use $T = 0.7$ without top-$k$ truncation.

\paragraph{Baselines.} 
We primarily compare \model with the following baselines. It is noteworthy that all baselines use the same LLM as the decoder. 
For a fair comparison, we report the results of Self-consistency, \model, and \model + Self-consistency with the same 5 rationales sampled from the decoder.
\begin{itemize}[wide, labelwidth=!, labelindent=15pt]
    \item \textit{CoT-Prompting.} CoT-Prompting~\citep{wei2022chain} is chain-of-thought prompting with greedy decoding.
    \item \textit{Self-consistency.} Self-consistency~\citep{wang2022self} is a decoding strategy to replace the greedy decoding strategy used in CoT-Prompting. Self-consistency sample from the LLM's decoder to generate a diverse set of rationales and determine the optimal answer by taking a majority vote.
\end{itemize}


\subsection{Main Results}\label{sec:main_results}

\begin{table*}[h]
\centering
\small
\setlength\tabcolsep{3pt}
    \centering
        \begin{tabular}{ccccccccc}
    \toprule
     & AddSub & MultiArith & Singleeq & Singleop & ASDiv & AQuA & SVAMP & GSM8K\\
    %  & AQuA & SVAMP & GSM8K
    \midrule
    CoT-prompting & 82.78 & 93.00 & 85.04 & 93.24 & 73.19 & 40.55 & 68.00 & 56.48 \\
    %  & 28.35 & 75.8 & 60.1
    Self-consistency & 90.63 & 94.17 & 89.17 & 93.59 & 77.72 & 38.19 & 75.70 & 58.85 \\
     % & 35.04 & 86.8 & 78.0
    \midrule
    \model & 92.15 & \textbf{95.50} & 92.51 & \textbf{93.78} & 75.52 & \textbf{44.09} & 74.60 & 61.56 \\
    %  & wait & wait & wait
    \model + Self-consistency & \textbf{97.22} & \textbf{95.50} & \textbf{94.09} & 93.59 & \textbf{79.63} & 41.34 & \textbf{80.10} & \textbf{61.94} \\
    %  & wait & wait & wait
    \bottomrule
    \end{tabular}
    \caption{Arithmetic reasoning accuracy by \model and \model + Self-consistency\citep{wang2022self} compared to Chain-of-Thought prompting\citep{wei2022chain} and Self-consistency. For a fair comparison, we use the same prompts as in \citep{wei2022chain}. Self-consistency, \model, and \model + Self-consistency use the same $5$ rationales sampled from the decoder. In our experiments, the threshold of Diversity Metrics is set to be top $40\%$， so only top $40\%$ predictions will be manually corrected. For each task, we report the median scores among 5 runs. }
    \label{tab:main-results-arithmetic}
\end{table*}



% We provide implementation details of baselines in Appendix \ref{apdx:baselines}. 




% We provide an ablation study in Section \ref{sec:ablation-number} to show that \model is generally robust to the number of rationales.

\paragraph{Arithmetic Reasoning} The results are shown in Tab.~\ref{tab:main-results-arithmetic}. \model generally improves the arithmetic reasoning performance at a large margin ($??$ on average). \model + Self-consistency further improves the arithmetic reasoning performance ($??$ on average). Especially for Singleeq and SVAMP, compared with CoT, the accuracy increased by 9.05$\%$ and 12.10$\%$, respectively.
% It also demonstrates that \model and self-consistency resolve different types of errors and play a complementary role to each other. 
% It also demonstrates that \model and self-consistency resolve different types of errors and play a complementary role to each other. 
% We provide an error case analysis in Sec.~\ref{subsection:error_case_study} to show more details about the error types that can be solved by the two methods.


\paragraph{Commonsense and Symbolic Reasoning} Tab.~\ref{tab:main-results-commonsense} shows the results on commonsense and symbolic reasoning tasks. Similarly, \model improves the performance and \model + Self-consistency further boosts it. 
For symbolic reasoning, we adopt the out-of-distribution (OOD) setting where the input prompt contains examples of 4-letters and 4-flips~ \citep{wang2022self} because this setting is more challenging. We do not adopt the in-distribution setting because GPT-3 can already achieve 100\% accuracy with the in-distribution setting as shown in \citet{wei2022chain}. Even in this difficult OOD setting, the gain of \model+Self-consistency is still quite significant compared to CoT-prompting and Self-consistency.


 
\begin{table}[htbp]
\centering
\small
\setlength\tabcolsep{3pt}
    \centering
    \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{Model} & \multicolumn{2}{c}{\textit{Commonsense}} & \multicolumn{2}{c}{\textit{Symbolic}} \\
    \cmidrule(r){2-3}
    \cmidrule(r){4-5}
     & CSQA & StraQA & Letter & Coinflip\\
    \midrule
    CoT-prompting & 72.32 & 60.13 & 49.20 & 81.40\\
    Self-consistency & 76.09 & \textbf{61.40} & 54.40 & \textbf{93.20}\\
    \midrule
    \model & 73.71 & 60.88 & 69.20 & 81.40\\
    \model + Self-consistency & \textbf{77.07} & 61.05 & \textbf{71.40} & \textbf{93.20}\\
    \bottomrule
    \end{tabular}
    \caption{Commonsense and symbolic reasoning accuracy by \model and \model + Self-consistency\citep{wang2022self} compared to Chain-of-Thought prompting\citep{wei2022chain} and Self-consistency. For a fair comparison, we use the same prompts as in \citep{wei2022chain}. Self-consistency, \model, and \model + Self-consistency use the same $5$ rationales sampled from the decoder. In our experiments, the threshold of Diversity Metrics is set to be top $40\%$. For each task, we report the median scores among 5 runs. }
    \label{tab:main-results-commonsense}
\end{table}

\begin{figure}%[ht]
\centering
\includegraphics[width=1.0\linewidth]{pic/numbers.png}
\caption{
Arithmetic reasoning accuracy by ~\model compared to Self-consistency\citep{wang2022self} under different number of decoded reasoning paths for Singleeq. For a fair comparison, both \model and Self-consistency use the same prompts as in \citet{wei2022chain}. Both \textcolor{magenta}{\model} and \textcolor{brown}{Self-consistency} use the same $5$ rationales sampled from the decoder. In our experiments, the threshold of Diversity Metrics is set to be top $40\%$. }
\label{fig:numbers}
\end{figure} 



% \begin{table}[htbp]
% \setlength\tabcolsep{3pt}
%     \centering
%     \begin{tabular}{cl  lllll'll}
%     \toprule
%     & Number & Self-consistency & \model \\
%     \midrule
%     & 5 & 93.42 & 91.39 \\
%     & 10 & 93.42 & 93,92 \\
%     & 15 & 92.41 & 94.42 \\
%     & 20 & 92.66 & 95.19 \\
%     & 25 & 93.16 & 95.70 \\
%     & 30 & 92.66 & 95.70 \\
%     & 35 & 92.66 & 96.20 \\
%     & 40 & 92.66 & 96.46 \\
%     \bottomrule
%     \end{tabular}
%     \caption{
%     Arithmetic reasoning accuracy by \model  compared to self-consistency\citep{wang2022self} under different number of rationales.
%     For fair comparison, both \model and self-consistency use the same prompts as in \citet{wei2022chain}. Both \model and self-consistency use the same decoding outputs as rationales.}
%     % 后面这个地方应该要换成图片，并且如果有钱的话，所有任务都可以做一下
%     \label{tab:number-of-reasoning-path}
% \end{table}

\subsection{Analysis of Whether Correcting Sub-logics Solves the Majority of Incorrect Rationales}
\label{subsection:error_case_study}

\begin{figure*}%[ht]
\centering
\includegraphics[width=1.0\linewidth]{pic/error_case_study.pdf}
\caption{
Illustration of error case analysis of Chain of Thought Prompting across tasks. Each task is represented by a pie chart. Each error type is represented by a color. The share of a color indicates the share of the error type.
}
\label{fig:error_case_study}
\end{figure*} 
We conduct experiments on twelve datasets to check whether correcting sub-logics solves the majority of incorrect rationales. 

We divide human correction into three types: modifying, adding, and deleting as shown in Sec. \ref{subsection:manual_correction}.
The percentage of each type across datasets is shown in Fig.~\ref{fig:error_case_study}.  Each error type is represented by a color.
\texttt{Unable to be manually corrected} means unsolvable problems that cannot be corrected within a single operation, including misinterpretation of the question, incorrect presentation, and incorrect formula.


For modifying, GPT-3 often makes errors when calculating polynomial calculations with decimal points, which account for a large part of manual correction.
For adding, GPT-3 often fails to convert the correct result of an operation to the units required by the question, which requires an adding of sub-logic to convert the calculation result.
For deletion, the model may be misled and thus output a redundant piece of logic, leading to the generation of incorrect answers, which could be fixed by deleting the redundant piece of logic.

Most of enhancement of Self-consistency comes from fixing unsolvable problem. Sampling a large set of reasoning paths and taking a majority vote helps the fix of misinterpretation of the question while making little help in fixing problems of calculation error.
The enhancement of \model comes from the manual correction of modifying, adding, and deleting.
The difference of error types that Self-consistency and \model solve may indicate that \model + Self-consistency achieves great performance because the major task performance enhancement of these two methods comes from fixing different kinds of errors.

\subsection{Additional Study}
\label{section:additional_study}

\paragraph{Diversity entropy is a strong method to rank the possibility for CoT predictions to be incorrect.}
\label{paragraph:ablation-diversity-metrics-ratio}

Diversity Entropy is a method to rank the possibility of each sample to be incorrect.
Here we perform a study using several thresholds of Diversity Entropy for manual correction to see if Diversity Entropy is an effective metric to rank the potential incorrect answers of CoT.
The results are shown in Fig.~\ref{fig:threshold}.
As the manual correction is labor-consuming and time-consuming, Diversity Entropy can help save time and labor because humans only need to check a small percentage of all samples.
\zefan{As Fig.~\ref{fig:threshold}, the performance stabilizes from $30\%$, so  we set the threshold to be top 40\% in all our experiments, and the threshold may not need to be frequently changed.}

\begin{figure}%[ht]
\centering
\includegraphics[width=1.0\linewidth]{pic/threshold.png}
\caption{
Results of different selections for the threshold value of diversity metrics. It shows the results of our \model respectively with 5\%, 10\%, 20\%, 30\%, 40\% and 50\% for Singleoq. For a fair comparison, we use the same prompts as in \citep{wei2022chain}. Results show that diversity metrics-based filtering is an efficient method to rank the possibility to be incorrect for the output of CoT predictions, and samples with incorrect output will be ranked higher than those without.
}
\label{fig:threshold}
\end{figure} 

\paragraph{Diversity Metrics Over Diverse Reasoning Paths}
\label{paragraph:diversity_metrics_over_diverse_reasoning_paths}

\begin{table}[h]
\small
\setlength\tabcolsep{4pt}
    \centering
    \begin{tabular}{c cccccc}
    \toprule
         & Singleop & ASDiv & AQuA & SVAMP & GSM8K\\
       \midrule
       UWA & 93.77 & 73.71 & 44.09 & 74.50 & 61.41 \\
       NWA & 93.77 & 73.71 & 40.94 & \textbf{74.60} & \textbf{61.56} \\
       \midrule
       UWS & 93.77 & 73.80 & 42.52 & 74.50 & 60.20 \\
       NWS & 93.42 & 73.37 & \textbf{44.88} & 71.30 & 59.21 \\
       \midrule
       UUS & \textbf{93.78} & \textbf{75.52} & 44.09 & \textbf{74.60} & \textbf{61.56} \\
       \bottomrule
    \end{tabular}
    \caption{Accuracy comparison of different answer aggregation strategies. The compared methods are listed as follows: UWA.: Unnormalized weighted average. NWA: Normalized weighted average. UWS: Unnormalized weighted sum. NWS: Normalized weighted sum. UUS: Unnormalized unweighted sum (Majority Vote). The threshold of Diversity Metrics is set to be top $40\%$. Results show that unnormalized unweighted sum generally outperforms other methods.}
    \label{table:aggregation}
\end{table}

Another interesting point that we want to explore is the aggregation strategies of Diversity Metrics. In practice, the Majority vote method of calculating the answer probability over all sampled reasoning paths is the same as taking unweighted sum. As described in \citet{wang2022self}, other selection of computing answer probability of $a$ over all sampled reasoning paths is to use unnormalized weighted average (UWA), normalized weighted average (NWA), unnormalized weighted sum (UWS), and normalized weighted sum (NWS). More details about the above calculation are provided at Sec.~\ref{appendix:diversity_metrics_over_diverse_reasoning_paths}. Tab.~\ref{table:aggregation} shows that unnormalized unweighted sum generally outperforms other methods

\subsection{Analysis of the Number of Sampled Rationales}
To illustrate the effect of the number of sampled rationales, we show the accuracy with respect to varying numbers of sampled paths (\ie, 1, 5, 10, 15, 20, 25, 30, 35, 40) in Fig.~\ref{fig:numbers}. \model generally outperforms self-consistency and benefit from increasing number of sampled rationales.

\subsection{Analysis of Balancing Cost and Utility}\label{sec:analysis_cost_utility}

\begin{table}[h]
\centering
\small
\setlength\tabcolsep{3pt}
    \centering
    % \begin{tabular}{cl  lllll'll}
        \begin{tabular}{ccccc}
    \toprule
    Method & Money & Time & Acc. & Utility \\
    \midrule
    CoT Prompting & $1$ & $1$ & 85.04 & 85.04 \\
    Self-consistency & $10$ & $10$ & 92.49 & 90.39 \\
    \model & $7$ & $7$ & 92.51 & 90.72 \\
    \model + Self-consistency & $7$ & $7$ & 94.09 & \textbf{92.29} \\
    Human & $10$ & $20$ & 95.00 & 92.19 \\
    \bottomrule
    \end{tabular}
    \caption{Analysis results on cost and utility based on the experiment results of Sec.~\ref{sec:main_results} and Fig.~\ref{fig:threshold} for Singleeq. The `Human' method denotes solving the problems with only human. Result shows that \model+Self-consistency generally outperform other methods with higher utility and less money cost.}
    \label{tab:utility-cost}
\end{table}

In Sec.~\ref{sec:framework}, we propose a Cost-utility Analysis Model based on In-context Learning (\cail). In this section, we will provide a detailed analysis for \cail based on the experiment results of Sec.~\ref{sec:main_results} and Fig.~\ref{fig:threshold}.
We set the price of sampling from the decoder for a dataset as $p_a$ and the time cost as $t_a$, which means using only an agent to solve the problem. The price of solving the problem with only humans is $p_s$ and the time cost is $t_s$. The price of manual correction for a dataset is $p_c$ and the time cost is $t_c$. $p_c$ and $t_c$ will be lower than $p_s$ and $t_s$ as manual correction requires less labor than solving the problem only by humans.

We consider five plans as follows: a naive plan that only requires GPT-3 for decoding only once, which will cost $p_a$ and $t_a$. A Self-Consistency plan that requires only agents without humans to sample from the decoder for 10 times, which will cost $10p_a$ and $10t_a$, as the GPT-3 API charges based on the number of tokens sampled from the decoder. . A \model plan to sample from decoder for 5 times, which will cost $5p_a + 0.4p_c$ and $5t_a + 0.4t_c$. A \model + Self-consistency plan to sample from the decoder for 5 times, which will cost the same as the \model plan. And a plan that requires only humans without agents, which will cost $p_s$ and $t_s$. Considering the user as the one who cares about getting solutions and not so much about time, then his utility function will be $u(a, t) = a^{1} t^{-0.01}$, where $a$ denotes the accuracy of the solution and $t$ is spent time. Based on practice, we set $p_a$ to $1$ unit of money, $p_c$ to $5$ unit of money and $p_s$ to $10$ units of money. As for time cost, we set $t_a$ to $1$ unit of time, $t_c$ to $5$ units of time and $t_s$ to $20$ units of time. The results are shown in Tab.~\ref{tab:utility-cost}. Result shows that \model+Self-consistency generally outperform other methods with higher utility and less money cost.
% The GPT-3 API charges according to the number of tokens to sample from the decoder. 
% Since \model requires to sample of 5 CoT predictions for each sample, the price of GPT-3 for \model is $5p_a$, and the price of a Self-consistency plan is $5p_a$. We assume that the price of manual correction for a dataset is $p_c$, and the price of manually solving the problems for the whole dataset is $p_s$ as manually correction is much more difficult than manually solving, causing much more consumption. \model requires to sample 5 CoT predictions for each sample and manual correction for $40\%$ of the CoT predictions, so the price of \model is $5p_a + 0.4p_h$. The price of \model without Diversity Entropy is $p_a + p_h$. And the price of a plan with only human is $p_s$.


